Quantifying Market Efficiency Impacts of Aggregated Distributed Energy Resources

We focus on the aggregation of distributed energy resources (DERs) through a profit-maximizing intermediary that enables participation of DERs in wholesale electricity markets. Particularly, we study the market efficiency brought in by the large-scale deployment of DERs and explore to what extent such benefits are offset by the profit-maximizing nature of the aggregator. We deploy a game-theoretic framework to study the strategic interactions between an aggregator and DER owners. The proposed model takes into account the stochastic nature of the DER supply. We explicitly characterize the equilibrium of the game and provide illustrative examples to quantify the efficiency loss due to the strategic incentives of the aggregator. Our numerical experiments illustrate the impact of uncertainty and amount of DER integration on the overall market efficiency.

==> equilibria.tex <==
%!TEX root = main.tex


{\proposition[Nash equilibrium characterization] All Nash equilibria $\v{x}^*$ satisfy 
\begin{equation*}x^*_i=F^{-1}_i\(\frac{\E\[\frac{\partial}{\partial x_i} u_i(d_i^0+C_i^\omega-x_i^*)\]+\rho}{\lambda_{\text{RT}}}\),\end{equation*}
for each $i=1,2,\dots,N$. }

\proof{For each prosumer $i$, the objective $\pi_i(x_i,\v{x}_{-i})$ is given by 
\begin{align*}
&\E \[u_i\(d_i^0+C^\omega_i-x_i\)\] + \rho x_i  \\
 & \qquad- \underbrace{\lambda_{\text{RT}} \E \[\frac{\(\sum_{j=1}^N (x_j-C^\omega_j)\)^+}{\sum_{j=1}^N  (x_j-C_j^\omega)^+} (x_i-C_i^\omega)^+ \]}_{\E[\phi_i(\v{x}(\rho),\v{C^\omega})]}.\end{align*}
 
Let $t^\omega_i:=\sum_{j\neq i} (x_j-C^\omega_j)$ and $s^\omega_i:=\sum_{j\neq i} (x_j-C_j^\omega)^+$. Then, we have
\begin{align*}
&\frac{\E[\phi_i(\v{x}(\rho),\v{C^\omega})]}{\lambda_{\text{RT}}}=\E \[\frac{\(t^\omega_i+x_i-C^\omega_i\)^+}{s^\omega_i+(x_i-C_i^\omega)^+} (x_i-C_i^\omega)^+ \] \\ 
&=  \int_{\omega \in \Xcal_i}\[\frac{t^\omega_i+x_i-C^\omega_i}{s^\omega_i+x_i-C_i^\omega} (x_i-C_i^\omega)\] f({\bf{C}}^\omega) d{\bf{C}}^\omega \\
& \qquad\qquad\qquad + \int_{\omega \notin \Xcal_i}\[0\] f({\bf{C}}^\omega) d{\bf{C}}^\omega.
\end{align*}
where $ \Xcal_i:=\{\omega\in\Omega: x_i > C_i^\omega, t^\omega_i> C_i^\omega-x_i\}$. By Leibniz integral rule
\begin{align*}
&\frac{1}{\lambda_{\text{RT}}}\frac{\partial \E[\phi_i(\v{x}(\rho),\v{C^\omega})] }{\partial x_i}=\\
& \int_{ \omega \in \Xcal_i} \[\frac{(s^\omega_i-t^\omega_i)(x_i-C_i^\omega)}{(s^\omega_i+x_i-C_i^\omega)^2}+ \frac{t^\omega_i+x_i-C^\omega_i}{s^\omega_i+x_i-C_i^\omega}  \] f({\bf{C}}^\omega) d{\bf{C}}^\omega.
\end{align*}
Next, by the  first-order necessary condition of optimality, 
\begin{align*}
&\frac{\E\[\frac{\partial}{\partial x_i} u_i(d_i^0+C_i^\omega-x_i^*)\]+\rho}{\lambda_{\text{RT}}}\\
&= \int_{ \omega \in \Xcal_i}\[ \underbrace{\frac{(s^\omega_i-t^\omega_i)(x^*_i-C_i^\omega)}{(s^\omega_i+x^*_i-C_i^\omega)^2}}_{\geq 0}+ \underbrace{\frac{t^\omega_i+x^*_i-C^\omega_i}{s^\omega_i+x^*_i-C_i^\omega}}_{>0}  \] f({\bf{C}}^\omega) d{\bf{C}}^\omega\\
&> 0 \implies \rho \neq - \E\[\frac{\partial}{\partial x_i} u_i(d_i^0+C_i^\omega-x_i^*)\],
\end{align*}
for each $i=1,\dots,N$. 
Define the intersection  
$$\Xcal:= \Xcal_1 \cap \Xcal_2 \cap \dots \cap \Xcal_N = \{\omega\in\Omega: x^*_i > C_i^\omega, i=1,\dots,N\}.$$
Next, for each $\omega \in \Xcal$, it holds $s^\omega_i=t^\omega_i$, which implies
\begin{align*}
&\int_{ \omega \in \Xcal}\[ \frac{(s^\omega_i-t^\omega_i)(x^*_i-C_i^\omega)}{(s^\omega_i+x^*_i-C_i^\omega)^2}+ \frac{t^\omega_i+x^*_i-C^\omega_i}{s^\omega_i+x^*_i-C_i^\omega} \] f({\bf{C}}^\omega) d{\bf{C}}^\omega\\
&= \int_{ \omega \in \Xcal}\[ 0+1\] f({\bf{C}}^\omega) d{\bf{C}}^\omega=\int_{ \omega \in \Xcal}\[1\] f({\bf{C}}^\omega) d{\bf{C}}^\omega.
\end{align*}
A Nash equilibrium is attained at the intersection of best responses, and hence, by the first-order condition,
\begin{align*}
&\frac{\E\[\frac{\partial}{\partial x_i} u_i(d_i^0+C_i^\omega-x_i^*)\]+\rho}{\lambda_{\text{RT}}}=  \int_{ \omega \in \Xcal}\[ 1\] f({\bf{C}}^\omega) d{\bf{C}}^\omega \\
&=\int_{0}^{x^*_{j \neq i}}\int_{0}^{x^*_i}\[1\] f({\bf{C}}^\omega)d{\bf{C}}^\omega\\
&=  \int_{0}^{x^*_{j \neq i}}\int_{0}^{x^*_i}\[1\] f({\bf{C}}^\omega)d{\bf{C}}^\omega  +  \int_{x^*_{j \neq i}}^{\bar{C}_{j \neq i}}\int_{0}^{x^*_j}\[0\] f({\bf{C}}^\omega)d{\bf{C}}^\omega\\
&= \int_{0}^{\bar{C}_{j \neq i}}\int_{0}^{x^*_j}\[1\] f({\bf{C}}^\omega)d{\bf{C}}^\omega=F_i(x_i^*),
\end{align*}
for  each $i=1,\dots,N$.\qed} 

%
{\example[Linear utilities]{If the utility function $u_i$ for each $i$ is of the following form: $u_i(d_i^0+C_i^\omega-x_i)=\gamma_i(d_i^0+C_i^\omega-x_i)$, then the Nash equilibrium is uniquely given by 
\begin{equation}x_i^*=F_i^{-1}\(\frac{\rho-\gamma_i}{\lambda_{\text{RT}}}\), \qquad i=1,2,\dots,N. \label{eq:NE1}\end{equation}

Plugging  into aggregator's problem, with $X_{\min}=0$, $\v{A}$'s payoff is 
$$\pi_{\v{A}}(\rho,\v{x}^*(\rho))= (\lambda_{\text{DA}}-\rho) \sum_{i=1}^N F_i^{-1}\(\frac{\rho-\gamma_i}{\lambda_{\text{RT}}}\).$$
If $F_i$ is uniform, then $F_i^{-1}\(\frac{\rho-\gamma_i}{\lambda_{\text{RT}}}\)$ is linear and increasing in $\rho$, which implies that $\pi_{\v{A}}(\rho,\v{x}^*(\rho))$ is quadratic and strictly concave in $\rho$, and the optimizer $\rho^*$ is uniquely given by solving $\frac{\partial \pi_{\v{A}}(\rho^*,\v{x}^*(\rho^*))}{\partial}=0$, leading to a unique Stackelberg equilibrium $(\v{x}^*,\rho^*)$. }
}
%


%{\proposition[Homogeneous Prosumers with Linear Utilities] Let $C_i^\omega=C^\omega$ and $u_i(d_i^0+C^\omega-x)=\gamma(d_i^0+C^\omega-x),$ for each $i=1,\dots,N$. Then, the Stackelberg equilibria are given by $(\rho^*,\v{x}^*)$, where
%\begin{itemize}[leftmargin=*]
%\item $\v{x}^*$ is the Nash equilibrium of the prosumers game $\Gcal_N$, which is uniquely given by
%\begin{equation*}x_i^*=F^{-1}(z(\rho^*)), \qquad i=1,\dots,N. \label{eq:NE2}\end{equation*}
%\item $\rho^*$ satisfies
%\begin{equation*}\frac{\partial F^{-1}\(z(\rho^*)\)}{\partial \rho}  + \(\frac{1}{\lambda_{\text{RT}}z(\rho^*)-\lambda_{\text{DA}}+\rho^*} \)F^{-1}\(z(\rho^*)\)= 0, \label{eq:SE}\end{equation*}
%where $z(\rho^*)=\frac{\rho^*-\gamma}{\lambda_{\text{RT}}}$.
%
%\end{itemize}}
%\subsection{Homogeneous Prosumers with Linear Utilities}
%Our result in Proposition \ref{prop.exist} guarantees the existence of an equilibrium, but does not reveal how that equilibrium behaves with various problem parameters. Towards that goal, we consider the prosumer-aggregator game with $N$ homogeneous prosumers, each with an identical energy capacity $C$, a nominal demand $d^0$, and a utility of consumption, given by
%$u(z):= \ln(1+z)$ for $z \geq 0$. 
%Given a wholesale electricity market price $\lambda$, call that game $\Gcal_h(\lambda)$. We characterize the equilibrium of $\Gcal_h (\lambda)$ in our next result that reveals the dependency of the outcome on the various problem parameters. We also exploit the result in the next section to analyze the resulting efficiency of the wholesale markets.
%
%
%We remark that accurately modeling the preferences of end-use customers in electricity consumption remains a challenging task. See \cite{feng} for a discussion. Logarithmic utility is commonly used in the economics literature \cite{shadow} for various commodities, and has recently found applications in the electricity market literature, e.g., in \cite{gao,sabita,mywork}. 
%
%To state our next result, we use the notation 
%$$ [z]_{z_{\min}}^{z_{\max}} := 
%\begin{cases}
%z_{\min}, & \text{if } z < z_{\min}, \\
%z_{\max}, & \text{if } z > z_{\max}, \\
%z, & \text{otherwise}
%\end{cases}
%$$
%for scalars $z, z_{\min}, z_{\max}$.
%
%\begin{proposition}[Homogeneous prosumers]
%Given a wholesale market price $\lambda$, the unique Stackelberg equilibrium of the prosumer-aggregator game $\Gcal_h(\lambda)$ is described by
%%
%\begin{align*}
%X^*(\rho) = N\(\bar{d}+C-\frac{1}{\rho}\), \ \
%\rho^* (\lambda) = \sqrt{\frac{ [\lambda]_{\lambda_{\min}}^{\lambda_{\max}} }{\bar{d}+C}}, 
%\end{align*}
%where $\bar{d}:=1+d^0$, and 
%\begin{align*}
%\lambda_{\min} := \frac{\bar{d}+C}{\[\bar{d}+C-(X_{\min} /N)\]^2}, \qquad
%\lambda_{\max} := \frac{\bar{d}+C}{[\bar{d}]^2 }.
%\end{align*}
% \label{prop:equilibrium}
%\end{proposition}
%%
%
%
%The equilibrium pair describes the total offered prosumers quantity $X^*$ as a function of the price $\rho$ announced by the aggregator and, the aggregator's price given the wholesale market price $\lambda$. When $\rho^*$ is high enough, prosumers sell their entire available generation. They prefer to consume the locally generated power, otherwise. The aggregator's offer price to the prosumers increases with the wholesale market price $\lambda$ and, when $\lambda$ is high enough,  the aggregator extracts the full supply capacities from the prosumers. The equilibrium is unique as \eqref{eq:concavity} holds for logarithmic utilities.
%
